DeepMix: Mobility-aware, Lightweight, and Hybrid 3D Object Detection for Headsets

Mobile headsets should be capable of understanding 3D physical environments to offer a truly immersive experience for augmented/mixed reality (AR/MR). However, their small form-factor and limited computation resources make it extremely challenging to execute in real-time 3D vision algorithms, which are known to be more compute-intensive than their 2D counterparts. In this paper, we propose DeepMix, a mobility-aware, lightweight, and hybrid 3D object detection framework for improving the user experience of AR/MR on mobile headsets. Motivated by our analysis and evaluation of state-of-the-art 3D object detection models, DeepMix intelligently combines edge-assisted 2D object detection and novel, on-device 3D bounding box estimations that leverage depth data captured by headsets. This leads to low end-to-end latency and significantly boosts detection accuracy in mobile scenarios. A unique feature of DeepMix is that it fully exploits the mobility of headsets to fine-tune detection results and boost detection accuracy. To the best of our knowledge, DeepMix is the first 3D object detection that achieves 30 FPS (an end-to-end latency much lower than the 100 ms stringent requirement of interactive AR/MR). We implement a prototype of DeepMix on Microsoft HoloLens and evaluate its performance via both extensive controlled experiments and a user study with 30+ participants. DeepMix not only improves detection accuracy by 9.1--37.3% but also reduces end-to-end latency by 2.68--9.15x, compared to the baseline that uses existing 3D object detection models.

==> accuracy-yongjie.tex <==
\subsection{Object Detection Accuracy in Static Scenario}
\label{sec:accuracy-static1}

\subsection{Object Detection Accuracy in Mobile Scenarios}
\label{sec:accuracy-mobile1}


\vspace{-0.2in}
\begin{figure}[!htp]
  \includegraphics[width=0.9\linewidth]{./figures/Scenario.pdf}
  \vspace{-0.1in}
  \caption{\small User mobility pattern test scenarios.}
  \label{fig:scenario}
  \vspace{-0.1in}
\end{figure}



\begin{table*}[!htp]
\centering
\footnotesize 
\begin{tabular}{c|c|cccccccc|c}
%  State & \multicolumn{2}{c}{$\delta_c$} & State & \multicolumn{2}{c}{$\delta_c$}    \\ 
%\hline
Methods & Input & & \multicolumn{6}{c}{mSPA@0.70} &  & average \\ \cline{3-10}   
 &  & table & chair & bottle & box & book & desk & bag & tv &  \\  
 \hline %\hline

% DSS~\cite{song2016deep}       & PointCloud  & 52.2 & 47.5 & 41.4 & 58.1 & 46.9 & 72.2 & 41.6 & 39.2 & 49.2      
% \\       
 COG~\cite{ren2016three}       & PC  & 67.2 & 34.3 & 59.1 & 61.1 & 42.2 & 62.5 & 36.9 & 47.1 & 51.5                       
 \\
VoteNet~\cite{qi2019deep}   & PC  & 49.6 & 46.1 & 52.7 & 54.3 & 46.1 & 57.1 & 38.2 & 45.9 & 48.6
\\

MLCVNet~\cite{DBLP:conf/cvpr/XieLWWZXW20} & PC  & 62.5 & 73.4 & 61.8 & 58.7 & 66.1 & \textbf{77.6} & 56.7 & \textbf{52.2} & 63.2        \\

F-PointNet~\cite{qi2017frustum} & RGBD  & 41.9 & 53.4 & 48.6 & 44.7 & 51.1 & 42.1 & 35.4 & 37.1 & 44.3              
\\

Trans3D~\cite{DBLP:conf/iccv/TangL19} & RGBD  & 58.5 & 66.2 & 54.3 & 51.4 & 57.2 & 62.6 & 48.5 & 41.3 & 63.2      
\\

 
% 3DoP~\cite{chen20153d}   & RGB & 52.7 & 37.2 & 46.2 & 28.3 & 37.4 & 59.2 & 44.1 & \textbf{59.6} & 45.8
% \\
Mono3D~\cite{DBLP:conf/cvpr/ChenKZMFU16} & RGB & 57.7 & 34.2 & 79.9 & 36.2 & 55.1 & 41.6 & 56.7 & 47.2 & 50.5
\\

AM3D~\cite{DBLP:conf/iccv/MaWLZOF19}   & RGB & 53.8 & 46.6 & 75.2 & 48.5 & 62.1 & 52.3 & 59.4 & 44.5 & 54.5
\\
$D^4LCN$~\cite{DBLP:conf/cvpr/DingHYWSLL20}& RGB & 52.7 & 72.6 & 67.4 & 64.7 & 59.3 & 54.6 & 71.2 & 46.5 & 61.1 
\\

\hline
DeepMix & RGB+D & \textbf{69.3} & \textbf{85.4} & \textbf{84.1} & \textbf{75.6} & \textbf{76.2} & 57.4 & \textbf{77.1} & 43.6 & \textbf{71.3}
\\
%\hline
\end{tabular}
\vspace{0.1in}
\caption{Class-wise mSPA@0.7 comparison of our system (\name) to state-of-the-art 3D object detection models.}
\label{mSPA results}
\vspace{-0.2in}
\end{table*}





\begin{table*}[!htp]
\centering
\footnotesize 
\begin{tabular}{c|c|cccccccc|c}
% \begin{tabular}{|c|c|m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}|c|}
%  State & \multicolumn{2}{c}{$\delta_c$} & State & \multicolumn{2}{c}{$\delta_c$}    \\ 
\hline

Methods & Input & & \multicolumn{6}{c}{3D IoU@0.25/0.5} &  & average \\ \cline{3-10}   
 &  & \centering table &\centering chair &\centering bottle &\centering box &\centering book &\centering desk &\centering bag &\centering tv &  \\    \hline %\hline

% DSS~\cite{song2016deep}       & PointCloud  & 50.4/11.2 & 60.6/9.3 & 42.5/6.7 & 57.6/- & 36.5/7.4 & 41.3/- & 43.2/4.3 & 31.5/7.4 & 45.5/5.8      
% \\       
COG~\cite{ren2016three}       & PC  & 47.3/2.6 & 39.3/- & 46.4/1.8 & 57.3/15.2 & 41.4/8.6 & 49.5/13.3 & 45.1/10.3 & 39.5/5.7 & 47.9/7.2                             
\\ 

VoteNet~\cite{qi2019deep}   & PC  & 56.2/23.6 & 45.5/22.2 & 67.2/18.3 & 52.4/22.6 & 47.2/23.8 & 48.6/14.2 & 54.3/18.5 & 41.9/19.2 & 51.6/21.7
\\ 
MLCVNet~\cite{DBLP:conf/cvpr/XieLWWZXW20} & PC  & 61.3/22.5 & \textbf{74.2}/27.6 & \textbf{68.2}/16.4 & 62.1/22.3 & 59.4/21.8 & 63.7/26.5 & 57.6/21.1 & 52.3/17.9 & 63.1/22.1                                 
\\
F-PointNet~\cite{qi2017frustum}   & RGBD & 45.5/11.2 & 37.5/17.3 & 44.2/9.5 & 31.6/17.5 & 49.6/14.3 & 38.5/- & 54.5/17.6 & 37.4/8.2 & 42.3/11.9
\\

Trans3D~\cite{DBLP:conf/iccv/TangL19} & RGBD & 52.3/13.5 & 38.4/- & 47.2/13.2 & 39.5/8.4 & 55.7/14.2 & 47.2/18.4 & 49.1/- & 37.2/12.9 & 45.8/10.1
\\

Mono3D~\cite{DBLP:conf/cvpr/ChenKZMFU16} & RGB & 59.3/11.2 & 52.4/9.5 & 47.3/8.6 & 65.3/13.2 & 48.2/11.8 & 67.5/21.5 & 48.6/5.2 & 54.5/16.4 & 55.4/10.7
\\

AM3D~\cite{DBLP:conf/iccv/MaWLZOF19}    & RGB & 65.9/14.9 & 71.2/11.3 & 62.7/16.3 & 57.8/10.7 & 53.4/19.1 & 49.2/12.5 & 51.7/11.2 & 57.9/12.9 & 58.7/13.6
\\
$D^4LCN$~\cite{DBLP:conf/cvpr/DingHYWSLL20} & RGB & 68.3/14.3 &  69.2/24.4 & 67.2/18.6 & 58.9/21.5 & \textbf{71.9}/12.7 & 62.3/14.3 & 56.6/9.6 & 57.2/11.7 & 63.9 /15.9
\\

\hline
DeepMix & RGB+D & \textbf{72.4/37.5} & 67.4/\textbf{24.4} & 63.1/\textbf{38.4} & \textbf{66.5/39.1} & 61.5/\textbf{29.5} & \textbf{72.1/33.2} & \textbf{65.8/46.5} & \textbf{61.2/31.8} & \textbf{67.4/37.2}
\\
%\hline
\end{tabular}
\vspace{0.1in}
\caption{Class-wise 3D IoU@0.25/0.5 comparison of our system (\name) and state-of-the-art 3D object detection models.}
\vspace{-0.3in}
\label{tab:3DIoU-static1}
\end{table*}






\begin{table*}[!htp]
\centering
\footnotesize 
\begin{tabular}{c|c|cccc|c}
% \begin{tabular}{|c|c|m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}|c|}
%  State & \multicolumn{2}{c}{$\delta_c$} & State & \multicolumn{2}{c}{$\delta_c$}    \\ 
%\hline

Methods & Input & \multicolumn{4}{c}{3D IoU@0.25(Scenario 1: speed@0.5/1/2 m/s)} & average \\ \cline{3-7}   
 & &\centering chair  &\centering bottle &\centering box  &\centering bag  &  \\    \hline %\hline

% DSS~\cite{song2016deep}       & PointCloud  & 50.4/11.2 & 60.6/9.3 & 42.5/6.7 & 57.6/- & 36.5/7.4 & 41.3/- & 43.2/4.3 & 31.5/7.4 & 45.5/5.8      
% \\       
COG~\cite{ren2016three}       & PC  &  27.6/21.5/3.1 & 37.5/8.6/- &  35.2/11.6/-  & 24.8/12.4/3.4  & 31.2/13.5/1.6                             
\\ 

VoteNet~\cite{qi2019deep}   & PC  &  34.7/24.2/5.1 & 44.2/11.3/-  & 42.1/18.4/6.2  & 37.5/12.1/6.8  & 39.6/17.6/4.5
\\ 
MLCVNet~\cite{DBLP:conf/cvpr/XieLWWZXW20} & PC  &  54.2/36.1/10.2 & 56.1/22.5/-  & 47.1/24.6/9.2 & 37.5/13.2/5.9 & 48.7/26.1/4.3                                 
\\
F-PointNet~\cite{qi2017frustum}   & RGBD &  28.6/13.6/3.4 & 36.5/14.3/-  & 24.1/16.6/2.1  & 25.6/12.9/7.8  & 28.7/14.3/3.3
\\

Trans3D~\cite{DBLP:conf/iccv/TangL19} & RGBD &  32.4/17.6/6.8 & 27.2/16.3/5.6  & 18.4/11.2/-  & 38.5/24.1/11.8  & 29.1/17.3/6.1
\\

Mono3D~\cite{DBLP:conf/cvpr/ChenKZMFU16} & RGB &  54.2/38.4/21.5 & 37.2/19.5/11.2  & 59.4/42.1/27.7  & 36.9/28.8/9.6  & 46.9/32.2/17.5
\\

AM3D~\cite{DBLP:conf/iccv/MaWLZOF19}    & RGB &  61.7/40.5/31.8 & 53.6/26.3/14.5  & 51.7/33.2/18.5  & 57.2/36.7/17.2  & 58.2/34.2/20.5
\\
$D^4LCN$~\cite{DBLP:conf/cvpr/DingHYWSLL20} & RGB &   59.7/47.2/33.8 & 51.2/22.4/18.5  & \textbf{64.1}/57.7/27.5  & 50.6/34.5/14.2  & 56.4/40.4/23.5 
\\

\hline
DeepMix & RGB+D &  \textbf{63.1}/\textbf{48.2}/\textbf{34.1} & \textbf{58.1/42.9/27.1} & 59.4/\textbf{42.6/31.8} & \textbf{57.9/34.2/24.9} & \textbf{60.5/41.9/29.4}
\\
%\hline
\end{tabular}
\vspace{0.1in}
\caption{Class-wise 3D IoU@0.25 comparison of our system to state-of-the-art 3D object detection methods under mobile scenario 1.}
\vspace{-0.3in}
\label{3DIoU results motion}
\end{table*}




\begin{table*}[!htp]
\centering
\footnotesize 
\begin{tabular}{c|c|cccc|c}
% \begin{tabular}{|c|c|m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}|c|}
%  State & \multicolumn{2}{c}{$\delta_c$} & State & \multicolumn{2}{c}{$\delta_c$}    \\ 
%\hline

Methods & Input & \multicolumn{4}{c}{3D IoU@0.25(Scenario 2: speed@0.5/1/2 m/s)} & average \\ \cline{3-7}   
 & &\centering chair  &\centering bottle &\centering box  &\centering bag  &  \\    \hline %\hline

% DSS~\cite{song2016deep}       & PointCloud  & 50.4/11.2 & 60.6/9.3 & 42.5/6.7 & 57.6/- & 36.5/7.4 & 41.3/- & 43.2/4.3 & 31.5/7.4 & 45.5/5.8      
% \\       
COG~\cite{ren2016three}     & PC  &  29.5/22.1/11.5 &  35.2/12.6/4.9 &  37.2/13.5/3.5  & 27.1/11.2/4.4  & 31.2/13.5/1.6                             
\\ 

VoteNet~\cite{qi2019deep}   & PC  &  36.1/21.5/3.7 & 41.2/13.2/5.2  & 42.6/16.7/7.1  & 39.2/11.7/7.7  & 39.7/15.7/5.9
\\ 
MLCVNet~\cite{DBLP:conf/cvpr/XieLWWZXW20} & PC  &  51.8/38.1/12.7 & 58.6/24.3/4.4  & 42.5/22.1/7.6 & 36.9/16.7/8.2 & 47.5/25.3/8.2                                
\\
F-PointNet~\cite{qi2017frustum}   & RGBD &  27.1/14.3/3.7 & 39.4/16.1/5.8  & 28.9/19.7/7.4  & 27.6/14.5/9.4  & 30.1/16.1/6.6
\\

Trans3D~\cite{DBLP:conf/iccv/TangL19} & RGBD &  32.1/16.6/8.4 & 36.7/19.2/11.2  & 26.6/17.4/6.8  & 44.2/27.1/12.6  & 34.9/20.1/9.8
\\

Mono3D~\cite{DBLP:conf/cvpr/ChenKZMFU16} & RGB &  57.4/41.7/25.6 & 42.1/17.6/13.5  & 58.9/45.2/19.8  & 42.5/29.6/13.3  & 50.2/33.5/18.1
\\

AM3D~\cite{DBLP:conf/iccv/MaWLZOF19}    & RGB &  \textbf{67.2}/46.8/36.4 & 59.4/32.7/19.7  & 60.4/37.2/22.5  & 55.4/38.2/14.8  & 60.6/38.7/23.4
\\
$D^4LCN$~\cite{DBLP:conf/cvpr/DingHYWSLL20} & RGB &   65.2/51.2/36.7 & 57.4/32.1/17.6  & \textbf{68.2}/51.3/23.8  & 52.4/36.8/13.8  & 60.8/42.9/22.9 
\\

\hline
DeepMix & RGB+D &  66.5/\textbf{58.2}/\textbf{47.4} & \textbf{77.5/63.2/35.4} & 62.2/\textbf{46.7/39.2} & \textbf{58.3/41.3/33.1} & \textbf{62.1/50.4/38.7}
\\
%\hline
\end{tabular}
\vspace{0.1in}
\caption{Class-wise 3D IoU@0.25 comparison of our system to state-of-the-art 3D object detection methods under mobile scenario 2.}
\vspace{-0.3in}
\label{3DIoU results motion 2}
\end{table*}

\begin{table*}[!htp]
\centering
\footnotesize 
\begin{tabular}{c|c|cccc|c}
% \begin{tabular}{|c|c|m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}m{1cm}|c|}
%  State & \multicolumn{2}{c}{$\delta_c$} & State & \multicolumn{2}{c}{$\delta_c$}    \\ 
%\hline

Methods & Input & \multicolumn{4}{c}{3D IoU@0.25(Scenario 3: speed@0.5/1/2m/s)} & average \\ \cline{3-7}   
 & &\centering chair  &\centering bottle &\centering box  &\centering bag  &  \\    \hline %\hline

% DSS~\cite{song2016deep}       & PointCloud  & 50.4/11.2 & 60.6/9.3 & 42.5/6.7 & 57.6/- & 36.5/7.4 & 41.3/- & 43.2/4.3 & 31.5/7.4 & 45.5/5.8      
% \\       
COG~\cite{ren2016three}     & PC  &  38.5/33.2/27.4 &  32.2/27.6/19.7 &  46.2/34.1/28.6  & 36.8/28.8/21.6 & 38.4/30.9/24.3                             
\\ 

VoteNet~\cite{qi2019deep}   & PC  &  48.4/35.5/29.2 & 52.1/43.2/24.6  & 48.5/36.7/28.2  & 45.2/30.2/18.1  & 48.6/36.4/25.1
\\ 
MLCVNet~\cite{DBLP:conf/cvpr/XieLWWZXW20} & PC  &  55.7/42.2/28.4 & 53.7/43.2/33.9  & 45.2/30.2/19.8 & 44.6/25.1/17.2 & 49.8/35.1/24.8                                 
\\
F-PointNet~\cite{qi2017frustum}   & RGBD &  32.8/21.3/17.6 & 35.2/25.9/21.2  & 25.6/14.1/8.9  & 41.8/32.4/19.6  & 33.9/23.4/16.8
\\

Trans3D~\cite{DBLP:conf/iccv/TangL19} & RGBD &  33.8/25.7/22.4 & 34.6/22.5/17.6  & 33.7/25.4/15.5  & 45.5/36.2/18.6  & 36.9/27.5/18.5
\\

Mono3D~\cite{DBLP:conf/cvpr/ChenKZMFU16} & RGB &  59.6/49.1/41.6 & 45.2/37.6/23.9  & 66.5/51.1/36.2  & 41.7/34.1/27.7  & 53.2/42.9/32.3
\\

AM3D~\cite{DBLP:conf/iccv/MaWLZOF19}    & RGB &  64.5/54.2/47.3 & 59.4/47.2/32.9  & 63.3/54.9/46.2  & 61.4/53.2/42.5  & 62.1/52.4/42.2
\\
$D^4LCN$~\cite{DBLP:conf/cvpr/DingHYWSLL20} & RGB &   65.3/49.2/41.7 & 54.8/47.3/39.2  & 64.7/56.8/48.9  & 53.6/48.6/39.5  & 59.6/50.5/42.3 
\\

\hline
DeepMix & RGB+D &  \textbf{78.3}/\textbf{69.7}/\textbf{61.4} & \textbf{73.5/74.2/52.7} & \textbf{68.7/58.9/51.2} & \textbf{64.5/68.4/49.8} & \textbf{71.2/61.8/53.8}
\\
%\hline
\end{tabular}
\vspace{0.1in}
\caption{Class-wise 3D IoU@0.25 comparison of our system to state-of-the-art 3D object detection methods under mobile scenario 3.}
\vspace{-0.3in}
\label{tab:3DIoU-m3}
\end{table*}









\guan{In order to have a better understanding of our system, we evaluate our system with other state-of-the-art 3D object detection methods under different use cases. In the evaluation, we chose CoG~\cite{ren2016three} , VoteNet~\cite{qi2019deep} and MLCVNet~\cite{DBLP:conf/cvpr/XieLWWZXW20} as the point cloud based 3D object detection methods; F-PointNet~\cite{qi2017frustum} and Trans3D~\cite{DBLP:conf/iccv/TangL19} as the RGBD based 3D object detection methods; Mono3D~\cite{DBLP:conf/cvpr/ChenKZMFU16}, AM3D~\cite{DBLP:conf/iccv/MaWLZOF19}, and $D^4LCN$~\cite{DBLP:conf/cvpr/DingHYWSLL20} as the monocular RGB based 3D object detection methods. All the methods are fine turning with SUN RGBD dataset~\cite{song2015sun}.} 



\subsubsection{Accuracy of 3D Object Detection}
\guan{The accuracy is an essential indicator of a 3D object detection method. We experiment to evaluate the 3D detection accuracy by using mSPA and 3D IoU metrics. Since the AR/MR headsets are usually used in dynamic environment, we design both static scenarios and mobile scenarios. In order to make the experiment have a fair environment for comparison in static scenarios, the input data of different methods are imported from the testing dataset which is mentioned in Section~\ref{Dataset}. In mobile scenarios, since the captures of camera are dynamic, we utilize the real-time captures (i.e., RGB, depth.) of device as the input of each method. And the user mobility pattern test cases are illustrated in Fig.~\ref{fig:scenario} and described below.}

\begin{itemize}
    \item Scenario 1: Parallel movement: The direction of user movement is perpendicular to the direction of the object, and the moving range is 2 meters.
    \item Scenario 2: Away/Close movement: The User move close/away to the object, and the moving range is 2 meters. 
    \item Scenario 3: Circling movement: The user moves around the object, the distance between the object and the user is 1 to 2 meters.
\end{itemize}
  

\guan{In static scenario, remarkably, our system achieves better overall performance than all the other methods under different object categories. In Table~\ref{mSPA results}, the average mSPA (mean Spatial Position Accuracy) of DeepMix reaches 71.3\% on our testing dataset, 3.5\% higher than the current state-of-the-art point cloud-based method, MLCVNet. Furthermore, for RGB-based 3D object detection methods, our methods are 10.2\% higher than the RGB-based method, $D^4LCN$. In Table~\ref{mSPA results}, our system reaches the highest mSPA in most of the object categories. However, our system cannot achieve the highest accuracy in the classes "desk" and "tv". After analyzing the detection results, we find that the hardware limitation of the system causes the low mSPA. When the system tries to collect the depth information of the detected objects, a minor part of the object, e.g., edge of the TV, legs of the desk, may not be perceived by the depth sensor. In summary, the inaccurate depth data leads to a decrease in mSPA. To have a better understanding of the system performance, we conduct experiments to evaluate the 3D IoU of the detection methods on our testing dataset. Table~\ref{3DIoU results} shows the 3D IoU of eight state-of-the-art 3D object detection methods. The results show that our system has the highest average 3D IoU. Especially when the threshold of 3D IoU is set to 0.5, the performance of our system is $1.6\times$ over state-of-the-art methods. It is found that cube-like objects, such as bottles, boxes, desks, and bags, usually get bigger improvements. The reason could be that the dimension of these objects can be calculated more accurately from the depth frame.}  

\guan{We also conduct experiment under different mobile scenarios, Table~\ref{3DIoU results motion} and Table~\ref{3DIoU results motion 2} shows the 3D IoU(@0.25) comparison under mobile scenario 1 and scenario 2 which is shown in Fig.~\ref{fig:scenario}. In mobile scenario 1, our system achieve the highest average 3D IoU under different object class. The results show that long end-to-end latency can cause the mismatch between objects and bounding boxes, for example, MLCVNet have $63.1\%$ 3D IoU(@0.25) in static scenario, and the 3D IoU is reduced to $48.7\%$ when the user moves at a speed of 0.5m/s. Moreover, the most of results in Table~\ref{3DIoU results motion 2} are better than the results from Table~\ref{3DIoU results motion}. After analysing the captures of different scenarios, we find  parallel movement can lead to larger displacement changes of the object on the image than Away/Close movement under the same moving speed. And higher Speed of displacement change can lead to larger dismatch between object and bounding boxes. Moreover, In Table~\ref{3DIoU results motion 3}, our system reaches the highest 3D IoU of different mobile scenarios. When user moves around the object, our system can capture and detect the object from different angles and get different detection results. By combining the detection results, the detection accuracy can be improved. } 

